Joint Optimization of Transmission and Propulsion in UAV-Assisted Communication Networks

The communication energy in a wireless network of mobile autonomous agents should be defined to include the propulsion energy as well as the transmission energy used to facilitate information transfer. We therefore develop communicationtheoretic and Newtonian dynamic models of the communication and locomotion expenditures of an unmanned aerial vehicle (UAV). These models are used to formulate a novel nonlinear optimal control problem (OCP) for arbitrary networks of autonomous agents. This is the first work to consider mobility as a decision variable in UAV networks with multiple access channels. Where possible, we compare our results with known analytic solutions for particular single-hop network configurations. The OCP is then applied to a multiple-node UAV network for which previous results cannot be readily extended. Numerical results demonstrate increased network capacity and communication energy savings upwards of 70% when compared to more naive communication policies.

==> Images/Tikz_Pic_IoTSim.tex <==
\begin{figure}[t!]
\centering{
\resizebox{\linewidth}{!}{
\begin{tikzpicture}[scale=0.7]
	%\draw[step=1cm,gray,ultra thin] (-2,-1) grid (12,5);

	\draw[blue, ultra thick,->] (0,3) -- (6,3);
   	\draw[blue, ultra thick,|-|] (-1,3) -- (11,3);
    \node[draw=none, align=center] at (-1,2.5) {$Q_\text{init}$};
    \node[draw=none, align=center] at (11,2.5) {$Q_\text{final}$};

    
	%Dashed distance interconnections
    %\draw[black,dotted, line width=0.4mm, ->] (2,4.8) -- (2,3.3);
	\draw[black,dashed, line width=0.4mm, ->] (0,0) -- (1.4,2.5);
   	\draw[black,dashed, line width=0.4mm, ->] (1,0) -- (1.7,2.5);
	\draw[black,dashed, line width=0.4mm, ->] (2,0) -- (2,2.5);
	\draw[black,dotted, line width=0.4mm, ->] (2,3) -- (7.5,0.2);

	% UAV
    \node[inner sep=0pt, align=center] (UAV) at (2,3)
    {\scalebox{1}[-1]{\includegraphics[angle=170,width=.1\textwidth]{Images/UAV_flying_wing_edit4}}};
    \node[draw=none, align=center] at (1.5,3.5) {$U_N$};

    % AP
    \node[inner sep=0pt, align=center] (AP) at (8,-0.5)
    {\includegraphics[width=.03\textwidth]{Images/Base_station}}; 
    \node[draw=none, align=center] at (9,-0.5) {AP \\ $(0,0)$};

	% Altitude Line
	\draw[gray, thick, <->] (8,0.1)--(8,2.9);
	\node[draw=none, align=center] at (8.5,1.5) {$a$};

	%Source nodes
    \node[inner sep=0pt, align=center] (AP) at (0,-0.5)
    {\includegraphics[width=.02\textwidth]{Images/IEC_Antenna_svg}}; 
       \node[inner sep=0pt, align=center] (AP) at (1,-0.5)
    {\includegraphics[width=.02\textwidth]{Images/IEC_Antenna_svg}}; 
       \node[inner sep=0pt, align=center] (AP) at (2,-0.5)
    {\includegraphics[width=.02\textwidth]{Images/IEC_Antenna_svg}}; 

	\node[draw=none, align=center] at (1,-1.8) {$U_1, \ldots, U_{N-1}$};
    \draw [
    ultra thick,
    decoration={
        brace,
        mirror,
        raise=0.5cm
    },
    decorate
] (-0.2,-0.5) -- (2.2,-0.5) ;

	%Ground
	\draw[RawSienna, line width=0.8mm] (-2,-1.1) -- (12,-1.1);
    
    %\node[draw=none, align=center] at (2.5,4.5) {$\varrho(t)$};

\end{tikzpicture}}}
\caption[Two node non-cooperative experimental set-up]{ Geometric configuration, shown in two dimensions, featuring a single relay $U_3$, an access point (AP) and $N$ source nodes. $U_3$ flies at an altitude $a=1000$\,m with no lateral displacement. Data links between nodes and for incoming data $\rho(t)$ are shown by dashed lines.}
    \label{fig:SimDiagram2}
\end{figure}

==> Images/Tikz_Pic_MultUAV.tex <==
\begin{figure}[t!]
\centering{
\resizebox{\linewidth}{!}{
\begin{tikzpicture}[scale=0.7]
	%\draw[step=1cm,gray,ultra thin] (-2,-1) grid (12,5);

	% UAV 1 trajectory
    \draw[ForestGreen, ultra thick] (-1,1.65) -- (11,1.65);
    \draw[blue, ultra thick,->] (0,3) -- (6,3);
   	\draw[blue, ultra thick,|-|] (-1,3) -- (11,3);
    \draw[ForestGreen, ultra thick,->] (0,1.65) -- (7,1.65);
    \node[draw=none, align=center] at (-1,2.3) {$Q_\text{init}$};
    \node[draw=none, align=center] at (11,2.3) {$Q_\text{final}$};
	% UAV 2 trajectory
    \draw[blue, ultra thick,->] (0,1.5) -- (6,1.5);
   	\draw[blue, ultra thick,|-|] (-1,1.5) -- (11,1.5);
    

	%Dashed distance interconnections
    %\draw[black,dotted, line width=0.4mm, ->] (2,4.8) -- (2,3.3);
	\draw[black,dotted, line width=0.4mm, ->] (2,3) -- (4.7,0.3);
	\draw[black,dotted, line width=0.4mm, ->] (2,1.5) -- (4.4,0.1);

	% UAV 1
    \node[inner sep=0pt, align=center] (UAV) at (1,1.5)
    {\scalebox{1}[-1]{\includegraphics[angle=170,width=.1\textwidth]{Images/UAV_flying_wing_edit4}}};
    \node[draw=none, align=center] at (0.5,2) {$U_1$};
    
    	% UAV 2
    \node[inner sep=0pt, align=center] (UAV) at (1,3)
    {\scalebox{1}[-1]{\includegraphics[angle=170,width=.1\textwidth]{Images/UAV_flying_wing_edit4}}};
    \node[draw=none, align=center] at (0.5,3.5) {$U_2$};

    % AP
    \node[inner sep=0pt, align=center] (AP) at (5,-0.5)
    {\includegraphics[width=.03\textwidth]{Images/Base_station}}; 
    \node[draw=none, align=center] at (6,-0.5) {$U_0$ \\ $(0,0)$};

	% Altitude Lines
    \draw[gray, thick, <->] (5,0.1)--(5,1.4);
	\draw[gray, thick, <->] (6.5,0.1)--(6.5,2.9);
	\node[draw=none, align=center] at (7.5,2.3) {$\sqrt[]{a_2^2 + \delta_2^2}$};
	\node[draw=none, align=center] at (5.5,0.8) {$a_1$};
    
	%Ground
	\draw[RawSienna, line width=0.8mm] (-2,-1.1) -- (12,-1.1);

\end{tikzpicture}}}
\caption{Geometric setup for simulations consisting of $N=1$ node (green), as per section~\ref{sec:singleNodeSim}, and $N=2$ nodes (blue) as per section~\ref{sec:TwoNodeSim}. Their speeds along these paths are variable and bounded. Tightening speed bounds adds a time parameterization to the paths, forming trajectory constraints. Nodes fly at altitudes $a_1=a_2=1000$\,m and lateral displacements of $\delta_2=0, \delta_2=1000$\,m.}
\label{fig:SimDiagram1}
\end{figure}

==> Images/Tikz_Pic_UAVChain.tex <==
\begin{figure}[t!]
\centering{
\resizebox{\linewidth}{!}{
\begin{tikzpicture}[scale=0.7]


    \node[draw=none, align=center] at (-2,1.5) {$Q_\text{init}$};
    \node[draw=none, align=center] at (12,1.5) {$Q_\text{final}$};
    
	% UAV trajectories
   	\draw[blue, ultra thick,|->] (-1,1.5) -- (2.8,1.5);
    \draw[blue, ultra thick,|->] (3,1.5) -- (6.8,1.5);
    \draw[blue, ultra thick,|->] (7,1.5) -- (11,1.5);

    % transmission lines
	\draw[black,dotted,line width=0.4mm, ->] (1.25,1.85) --   (4.75,1.85);
	\draw[black,dotted,line width=0.4mm, ->] (6.25,1.85) --   (8.75,1.85);
	\draw[black,dotted,line width=0.4mm, ->] (9.25,1.1) --   (10.8,0.1);

	% UAV 1
    \node[inner sep=0pt, align=center] (UAV) at (0,1.5)
    {\scalebox{1}[-1]{\includegraphics[angle=170,width=.1\textwidth]{Images/UAV_flying_wing_edit4}}};
    \node[draw=none, align=center] at (0.5,1) {$U_1$};
    
	% UAV 2
    \node[inner sep=0pt, align=center] (UAV) at (5,1.5)
    {\scalebox{1}[-1]{\includegraphics[angle=170,width=.1\textwidth]{Images/UAV_flying_wing_edit4}}};
    \node[draw=none, align=center] at (5.5,1) {$U_2$};
    
    % UAV 3
    \node[inner sep=0pt, align=center] (UAV) at (9,1.5)
    {\scalebox{1}[-1]{\includegraphics[angle=170,width=.1\textwidth]{Images/UAV_flying_wing_edit4}}};
    \node[draw=none, align=center] at (10,1) {$U_3$};

    % AP
    \node[inner sep=0pt, align=center] (AP) at (11,-0.5)
    {\includegraphics[width=.03\textwidth]{Images/Base_station}}; 
    \node[draw=none, align=center] at (12,-0.5) {$U_0$ \\ $(0,0)$};

	% Altitude Lines
%     \draw[gray, thick, <->] (5,0.1)--(5,1.4);
% 	\node[draw=none, align=center] at (5.5,0.8) {$a_1$};
    
	%Ground
	\draw[RawSienna, line width=0.8mm] (-2,-1.1) -- (12,-1.1);

 \end{tikzpicture}}}
\caption{Geometric setup for simulations consisting of $N=1$ node (green), as per section~\ref{sec:singleNodeSim}, and $N=2$ nodes (blue) as per section~\ref{sec:TwoNodeSim}. Their speeds along these paths are variable and bounded. Tightening speed bounds adds a time parameterization to the paths, forming trajectory constraints. Nodes fly at altitudes $a_1=a_2=1000$\,m and lateral displacements of $\delta_2=0, \delta_2=1000$\,m.}
\label{fig:SimDiagram1}
\end{figure}
